When Two Choices Are not Enough: Balancing at Scale in Distributed Stream Processing

Carefully balancing load in distributed stream processing systems has a fundamental impact on execution latency and throughput. Load balancing is challenging because real-world workloads are skewed: some tuples in the stream are associated to keys which are significantly more frequent than others. Skew is remarkably more problematic in large deployments: more workers implies fewer keys per worker, so it becomes harder to "average out" the cost of hot keys with cold keys. We propose a novel load balancing technique that uses a heaving hitter algorithm to efficiently identify the hottest keys in the stream. These hot keys are assigned to $d \geq 2$ choices to ensure a balanced load, where $d$ is tuned automatically to minimize the memory and computation cost of operator replication. The technique works online and does not require the use of routing tables. Our extensive evaluation shows that our technique can balance real-world workloads on large deployments, and improve throughput and latency by $\mathbf{150\%}$ and $\mathbf{60\%}$ respectively over the previous state-of-the-art when deployed on Apache Storm.

==> applications.tex <==
% !TEX root =  ../main.tex
\section{Applications}
\label{sec:applications}



==> notes.tex <==
% !TEX root =  ../main.tex
\section{Notes}
\begin{enumerate}
\item Load balancing in streams is an important issue when input distribution of keys is skewed
\begin{enumerate}
\item Current solutions do not work for different reasons (key grouping, shuffle grouping)
\item Hasn’t been studied well so far
\item Setting is Storm-like (no key identity in PE, no key migration possible)
\end{enumerate}
\item We propose to use PoTC to address the issue (nothing new here)
\begin{enumerate}
\item PoTC with “sticky” key grouping would give already good results (David’s simulations + proofs)
\item However PoTC can’t be used out of the box with multiple sources because there is a coordination problem (need to remember and have consensus on which of the choices is taken)
\end{enumerate}
\item We propose partial key grouping (``key splitting'') to address this issue (needs additional merge phase like shuffle grouping)
\begin{enumerate}
\item This requires a slightly different programming paradigm, which however has many applications (word count, naive bayes, sketches, SPDT)
\item We show that it works even better than normal PoTC (proof? and simulations)
\item Does not require coordination among sources (but requires load estimation)
\end{enumerate}
\item We propose local load estimation at the sources in a practical scenario
\begin{enumerate}
\item Compare with omniscient oracle (simulations)
\item Assess if some lightweight form of communication with destinations is useful (?) (simulations?)
\end{enumerate}
\item If the number of destinations/bins B are too many the load is unbalanced anyway
\begin{enumerate}
\item Key splitting helps in this case (explore power of d choices for $d>2$)
\end{enumerate}
\item We modify Storm to implement partial key grouping
\begin{enumerate}
\item Tests on live system
\item Release code
\end{enumerate}
\end{enumerate}

\section{Naming Conventions}

\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{l p{0.7\columnwidth}}
Partition		&	a division of the stream into sub-streams \\
Grouping		&	see Partition \\
Sub-Stream	&	a portion of the stream created by a partition \\
Message		&	an element of a stream, composed by a Key-Value pair \\
Tuple		&	see Message \\
Key			&	part of a Message that represents its identity \\
Stream		&	an infinite sequence of keyed messages \\
Key splitting	&	assigning a key to multiple (2) \peis \\
Power of both choices	&	see Key splitting \\
Static \potc	&	power of two choices \emph{without} key splitting \\
\end{tabular}
\end{center}
\label{default}
\end{table}%

